Signals of composite particles at the LHC

Composite particles generated by an unknown strong dynamics can be responsible for the ElectroWeak Symmetry Breaking (EWSB) and can substitute the Standard Model (SM) Higgs boson in keeping perturbative unitarity in the longitudinal WW scattering up to a cut-off \Lambda\approx 4\pi v. These new states can be sufficiently light to be observed at the Large Hadron Collider (LHC) and they can even be the first manifestation of new physics at the LHC. Their couplings among themselves and with the SM particles, can be described using reasonable effective Lagrangians and Chiral Perturbation Theory. In the first part of this thesis different possibilities for a strongly interacting EWSB are discussed in details with particular attention to the roles of unitarity in the longitudinal WW scattering and of ElectroWeak Precision Tests (EWPT). Higgsless models with composite vectors and scalars, based on the SU(2)_{L}\times SU(2)_{R}/SU(2)_{L+R} custodial symmetry, are discussed in the context of ElectroWeak Chiral Lagrangians and the phenomenology of the pair productions is studied for the high energy and high luminosity phase of the LHC. In the second part of the thesis the possible signals of single particle production at the early LHC, with 7 TeV of center of mass energy and 1-5 fb^{-1} of integrated luminosity, are treated with a phenomenological Lagrangian approach. The final states containing at least one photon emerge as the most promising channels for an early discovery already with tens of inverse picobarns of integrated luminosity. Finally, in the last part of this work, the role of a composite iso-singlet vector in Dark Matter models is discussed and the related LHC phenomenology is studied, giving particular attention to the Z\gamma final state.

==> 07_Notations.tex <==
%NOTATIONS AND CONVENTIONS
\chapter*{Notations and conventions}\l{notations}
\markboth{{\scshape Notations and conventions}}{{\scshape Notations and conventions}}
\addcontentsline{toc}{chapter}{Notations and conventions}
